FINESSE: A Versatile Beamline for Fundamental Interactions with Neutrons at the European Spallation SourcE

FINESSE (A Versatile Beamline for \textbf{F}undamental \textbf{I}nteractions with \textbf{N}eutrons at the \textbf{E}uropean \textbf{S}pallation \textbf{S}ourc\textbf{E}) is a proposed versatile beamline for fundamental interactions with neutrons at the European Spallation Source. Building on the HIBEAM design studies, FINESSE extends the original concept into a dual-guide beamline capable of operating either in a high-flux configuration or in a low-background configuration within a single ESS beam port. The high-flux branch is optimized for rare-process searches, including neutron--antineutron oscillations, neutron--sterile-neutron transitions, axion-like-particle searches, neutron charge measurements, and rare neutron decays. The low-background branch is designed for precision measurements requiring strong suppression of prompt and line-of-sight backgrounds, with a cryogenic neutron electric-dipole-moment experiment used as a benchmark case. A baseline exchangeable-guide concept has been developed in which only short guide sections inside the ESS bunker are exchanged, while the upstream extraction system and chopper positions remain fixed. A staged implementation, Short FINESSE, would use the upstream section of the high-flux beamline together with a compact magnetically controlled experimental region, enabling an early physics and R\&D programme before completion of the full facility. This paper summarizes the scientific case, beamline concept, guide simulations, chopper and timing system, magnetic-field control, detector developments, and staged implementation strategy. FINESSE would establish a long-term particle-physics infrastructure at ESS, providing a beamline for both discovery-driven searches and precision neutron measurements throughout the lifetime of the facility.

==> author_formatting.tex <==
\usepackage{etoolbox}

\makeatletter

\newcounter{affilctr}
\newbool{firstauthor}
\booltrue{firstauthor}

\newcommand{\AffilList}{}
\newcommand{\AuthorList}{}
\newcommand{\CurrentAffilNum}{}
\newcommand{\AffilNumListResult}{}

\newcommand{\DeclareAffiliation}[2]{%
  \csdef{affiltext@#1}{#2}%
}

\newcommand{\GetAffilNum}[1]{%
  \ifcsdef{affilnum@#1}{%
    \edef\CurrentAffilNum{\csuse{affilnum@#1}}%
  }{%
    \stepcounter{affilctr}%
    \csxdef{affilnum@#1}{\arabic{affilctr}}%
    \edef\CurrentAffilNum{\arabic{affilctr}}%
    \edef\temp{%
      \noexpand\gappto\noexpand\AffilList{%
        \noexpand\par
        \CurrentAffilNum.\space
        \csuse{affiltext@#1}%
      }%
    }%
    \temp
  }%
}

\newcommand{\BuildAffilNumList}[1]{%
  \begingroup
  \def\AffilNums{}%
  \newbool{firstaffil}%
  \booltrue{firstaffil}%
  \renewcommand*{\do}[1]{%
    \GetAffilNum{##1}%
    \ifbool{firstaffil}{%
      \xdef\AffilNums{\CurrentAffilNum}%
      \boolfalse{firstaffil}%
    }{%
      \xdef\AffilNums{\AffilNums,\CurrentAffilNum}%
    }%
  }%
  \docsvlist{#1}%
  \xdef\AffilNumListResult{\AffilNums}%
  \endgroup
}

\newcommand{\AddAuthor}[2]{%
  \BuildAffilNumList{#2}%
  \ifbool{firstauthor}{%
    \edef\temp{%
      \noexpand\gappto\noexpand\AuthorList{%
        #1\noexpand\textsuperscript{\AffilNumListResult}%
      }%
    }%
    \boolfalse{firstauthor}%
  }{%
    \edef\temp{%
      \noexpand\gappto\noexpand\AuthorList{%
        ,\space #1\noexpand\textsuperscript{\AffilNumListResult}%
      }%
    }%
  }%
  \temp
}

\newcommand{\PrintAuthors}{\AuthorList}
\newcommand{\PrintAffiliations}{{\AffilList}}

% Corresponding author marker + text
\newcommand{\corrauthormarker}{*}
\newcommand{\corrauthortext}{}

\newcommand{\SetCorrespondingAuthor}[1]{%
  \gdef\corrauthortext{Corresponding author: #1}%
}

\newcommand{\AddAuthorCorr}[2]{%
  \BuildAffilNumList{#2}%
  \ifbool{firstauthor}{%
    \edef\temp{%
      \noexpand\gappto\noexpand\AuthorList{%
        #1\noexpand\textsuperscript{\corrauthormarker,\AffilNumListResult}%
      }%
    }%
    \boolfalse{firstauthor}%
  }{%
    \edef\temp{%
      \noexpand\gappto\noexpand\AuthorList{%
        ,\space #1\noexpand\textsuperscript{\corrauthormarker,\AffilNumListResult}%
      }%
    }%
  }%
  \temp
}

\makeatother
